Dynamic Grasping with a Learned Meta-Controller

Grasping moving objects is a challenging task that requires multiple submodules such as object pose predictor, arm motion planner, etc. Each submodule operates under its own set of meta-parameters. For example, how far the pose predictor should look into the future (i.e., look-ahead time) and the maximum amount of time the motion planner can spend planning a motion (i.e., time budget). Many previous works assign fixed values to these parameters; however, at different moments within a single episode of dynamic grasping, the optimal values should vary depending on the current scene. In this work, we propose a dynamic grasping pipeline with a meta-controller that controls the look-ahead time and time budget dynamically. We learn the meta-controller through reinforcement learning with a sparse reward. Our experiments show the meta-controller improves the grasping success rate (up to 28% in the most cluttered environment) and reduces grasping time, compared to the strongest baseline. Our meta-controller learns to reason about the reachable workspace and maintain the predicted pose within the reachable region. In addition, it assigns a small but sufficient time budget for the motion planner. Our method can handle different objects, trajectories, and obstacles. Despite being trained only with 3-6 random cuboidal obstacles, our meta-controller generalizes well to 7-9 obstacles and more realistic out-of-domain household setups with unseen obstacle shapes.

==> sections/limitations.tex <==
\mysection{Limitations}
We are not able to provide real-world experiments. However, we think that the sim2real gap of this work is minimal, and the performance gain from the meta-controller will be consistent regardless of the sim2real gap. There are several reasons for it. (1) The largest gap when transferring to the real robot is the vision system that estimates the object poses and bounding box dimensions. Recent perception systems such as DOPE~\cite{tremblay2018deep} and Gen6D~\cite{liu2022gen6d} can obtain such information fast and reliably. We also add significant Gaussian noises to the poses and bounding box dimensions to account for such perception errors. Given the same magnitude, pure random noise is more challenging than noise from realistic perception systems with fixed observation-to-noise mapping. (2) Given the estimated poses and bounding box dimensions, there is no sim2real gap in other components of our pipeline, such as object pose predictor, grasp planner, motion planner, and the meta-controller. (3) Our simulated environment is under realistic timing. Time spent in all submodules is compensated with the target object motion and we retime the planned arm motion to make sure it matches the real-robot speed.
